The variety of extreme blazars in the AstroSat view

Extreme blazars have exceptionally hard intrinsic X-ray/TeV spectra and extreme peak energies in their spectral energy distribution (SED). Observational evidence suggests that the non-thermal emission from extreme blazars is typically non-variable. We aim to explore X-ray and GeV observational features of a variety of extreme blazars and also aim to test the applicability of various blazar emission models that could explain the very hard TeV spectra. We perform X-ray analysis of AstroSat and Swift-XRT data, along with gamma-ray data from Fermi-LAT, for sources; 1ES 0120+340, RGB J0710+591, 1ES 1101-232, 1ES 1741+196 and 1ES 2322-409. We employ three models: 1) a steady-state one-zone synchrotron-self-Compton (SSC) code, 2) another leptonic scenario of co-accelerated electrons and protons on multiple shocks, applied only on the extreme-TeVsources and 3) a one-zone hadro-leptonic (OneHaLe) code. The hadro-leptonic code is used twice to explain the gamma-ray emission process: proton synchrotron and synchrotron emission of secondary pairs. Our X-ray analysis provides well-constrained estimates of the synchrotron peak energies for both 1ES0120+340 and 1ES1741+196. The multi-epoch X-ray and GeV data reveal spectral and flux variabilities in RGB J0710+591 and 1ES 1741+196, even on time scales of days to weeks. As anticipated, the one-zone SSC model adequately reproduces the SEDs of regular HBLs but encounters difficulties in explaining the hardest TeV emission. Hadronic models offer a reasonable fit to the hard TeV spectrum, though with the trade-off of requiring extreme jet powers. On the other hand, the lepto-hadronic scenario faces additional challenges in fitting the GeV spectra of extreme-TeV sources. Finally, e-p co-acceleration scenario naturally accounts for the observed hard electron distributions and effectively matches the hardest TeV spectrum of RGB J0710+591 and 1ES 1101-232.

==> figures/1741_spectrum <==
set terminal qt size 550,1000 enhanced font "verdana,14"

set macros
set key left Left reverse nobox
set bars small
unset logscale
set logscale y
set style fill solid 1.0

# Margins for each row resp. column
MARGIN1 = "set tmargin at screen 0.99; set bmargin at screen 0.68"
MARGIN2 = "set tmargin at screen 0.68; set bmargin at screen 0.37"
MARGIN3 = "set tmargin at screen 0.37; set bmargin at screen 0.06"
MARGINA = "set lmargin at screen 0.18; set rmargin at screen 0.99" 

# x- and ytics for each row resp. column
#XTICS = "set xtics 1e-1,1e1,1e13; set format x '%.0e'; set mxtics 10; set xlabel '{/Symbol n} [Hz]'" #
XTICS = "set xtics 10,3,28; set format x '%g'; set mxtics 3; set xlabel 'log({/Symbol n} [Hz])'; set xlabel offset 0,0.5" #
NOXTICS = "set xtics add (''10,''13,''16,''19,''22,''25,''28); set mxtics 3; unset xlabel"
X2TICS = "set x2tics ('10'10,'13'13,'16'16,'19'19,'22'22,'25'25,'28'28); set x2tics offset 0.0,0.0; unset x2label"
NOX2TICS = "unset x2tics; unset x2label"

#YTICS1 = "set format y '%g'; set ylabel '{/Symbol n}F_{/Symbol n} [erg/cm^{2}/s]'; set yrange [9.5e-13:3.0e-9] noreverse; set mytics 10; set ylabel offset 0,0" 
#YTICS1 = "set format y '%g'; set ylabel '{/Symbol n}F_{/Symbol n} [erg/cm^{2}/s]'; set yrange [4e-13:1.1e-8] noreverse; set mytics 10; set ylabel offset 0,0" #deabsorbed, MWL
YTICS1 = "set format y '%g'; set ylabel '{/Symbol n}F_{/Symbol n} [erg/cm^{2}/s]'; set ytics 1e-13,1e1,1e-8; set mytics 10; set ylabel offset 0.6,0" #deabsorbed
NOYTICS = "unset ytics; set ytics add (''1e-12,''1e-11,''1e-10,''1e-9); set mytics 10; unset ylabel"

#UVOTLABEL = "unset label; set label 1 at 57187.5,15.00 'Swift/UVOT'" #font 'verdana,18'"
#ATOMLABEL = "unset label; set label 2 at 57187.5,14.60 'ATOM'" #font 'verdana,18'"

#ARROWSHESS = "set arrow 1 from 57157.877,0e-7 to 57157.877,1.5e-10 ls -1 nohead; set arrow 2 from 57160.954,0e-7 to 57160.954,1.5e-10 ls -1 nohead; set arrow 3 from #57164.956,0e-7 to 57164.956,1.5e-10 ls -1 nohead; set arrow 4 from 57220.844,0e-7 to 57220.844,1.5e-10 ls -1 nohead"

NOARROWS = "unset arrow"

LABEL3 = "unset label; set label 1 at graph 0.60,0.92 '1ES 1741+196' font 'verdana,12' tc rgb '#000000'; set label 2 at graph 0.60,0.85 'archival data' font 'verdana,12' tc rgb '#000000'"# rotate by 45"
LABELN1 = "unset label; set label 1 at graph 0.60,0.92 'contemp. data (1)' font 'verdana,12' tc rgb '#000000'"# rotate by 45"
LABELN2 = "unset label; set label 1 at graph 0.60,0.92 'contemp. data (2)' font 'verdana,12' tc rgb '#000000'"# rotate by 45"
NOLABEL = "unset label"


set multiplot layout 1,3 rowsfirst

@MARGINA; @MARGIN1
@NOXTICS; @NOX2TICS
@YTICS1
@NOARROWS; @LABEL3
plot [12:29][2e-13:5e-11] \
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::2::2 u (log10($1)):2:3 w filledcu lc rgb '#eeeeee' lw 1 title "",\
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::0::0 u (log10($1)):3:4 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::1::1 u (log10($1)):(1.5*$3):(0):(0.5*$3-$3) w vector lc 0 lw 2 title "",\
"SED_data/1ES1741+196/XRT_2012-13" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/XRT2020" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/UVOT" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/MAGIC" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/VERITAS" u (log10($1)):4:5 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/WISE" u (log10($1)):2 pt 7 lc 0 lw 2 title "",\
"steadystate/nFn_1741_l.dat" u (log10($1)):2 w l lc 7 lw 2 title "",\
"onehale/1741_1/Total_Power_old_lm.dat" u (log10($1)):3 w l lc 6 lw 2 dt (10,10) title "",\
"onehale/1741_1/Total_Power_old_hm.dat" u (log10($1)):3 w l lc 4 lw 2 dt (10,10,3,7) title "",\
"zech_model/HG_Costamante.dat" u (log10($1/(1+(0.084-0.184)))):($2*9.0) w l lc 0 lw 1 dt 1 title ""

#"SED_data/1ES1741+196/Fermi.dat" every :::2::2 u (log10($1)):2:3 w filledcu lc rgb '#dddddd' lw 1 title "",\
#"SED_data/1ES1741+196/Fermi.dat" every :::0::0 u (log10($1)):3:4 w yerrorbars pt 7 lc 8 lw 2 title "",\
#"SED_data/1ES1741+196/Fermi.dat" every :::1::1 u (log10($1)):(1.5*$3):(0):(0.5*$3-$3) w vector lc 8 lw 2 title "",\
#"SED_data/1ES1741+196/LAXPC_SED1_rebinned" u (log10($1)):2:3 w yerrorbars pt 7 lc 8 lw 2 title "",\
#"SED_data/1ES1741+196/SXT_SED1_rebinned" u (log10($1)):2:3 w yerrorbars pt 7 lc 8 lw 2 title "",\


@MARGINA; @MARGIN2
@NOXTICS; @NOX2TICS
@YTICS1
@NOARROWS; @LABELN1
plot [12:29][2e-13:5e-11] \
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::2::2 u (log10($1)):2:3 w filledcu lc rgb '#eeeeee' lw 1 title "",\
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::0::0 u (log10($1)):3:4 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::1::1 u (log10($1)):(1.5*$3):(0):(0.5*$3-$3) w vector lc 0 lw 2 title "",\
"SED_data/1ES1741+196/XRT_2012-13" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/XRT2020" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/UVOT" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/MAGIC" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/VERITAS" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/WISE" u (log10($1)):2 pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/Fermi.dat" every :::2::2 u (log10($1)):2:3 w filledcu lc rgb '#dddddd' lw 1 title "",\
"SED_data/1ES1741+196/Fermi.dat" every :::0::0 u (log10($1)):3:4 w yerrorbars pt 7 lc 8 lw 2 title "",\
"SED_data/1ES1741+196/Fermi.dat" every :::1::1 u (log10($1)):(1.5*$3):(0):(0.5*$3-$3) w vector lc 8 lw 2 title "",\
"SED_data/1ES1741+196/LAXPC_SED1_rebinned" u (log10($1)):2:3 w yerrorbars pt 7 lc 8 lw 2 title "",\
"SED_data/1ES1741+196/SXT_SED1_rebinned" u (log10($1)):2:3 w yerrorbars pt 7 lc 8 lw 2 title "",\
"steadystate/nFn_1741_1.dat" u (log10($1)):2 w l lc 7 lw 2 title "",\
"onehale/1741_1/Total_Power_lm.dat" u (log10($1)):3 w l lc 6 lw 2 dt (10,10) title "",\
"onehale/1741_1/Total_Power_hm.dat" u (log10($1)):3 w l lc 4 lw 2 dt (10,10,3,7) title "",\
"zech_model/HG_Costamante.dat" u (log10($1/(1+(0.084-0.184)))):($2*9.0) w l lc 0 lw 1 dt 1 title ""

@MARGINA; @MARGIN3
@XTICS; @NOX2TICS
@YTICS1
@NOARROWS; @LABELN2
plot [12:29][2e-13:5e-11] \
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::2::2 u (log10($1)):2:3 w filledcu lc rgb '#eeeeee' lw 1 title "",\
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::0::0 u (log10($1)):3:4 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/Fermi_10_11.dat" every :::1::1 u (log10($1)):(1.5*$3):(0):(0.5*$3-$3) w vector lc 0 lw 2 title "",\
"SED_data/1ES1741+196/XRT_2012-13" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/XRT2020" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/UVOT" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/MAGIC" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/VERITAS" u (log10($1)):2:3 w yerrorbars pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/WISE" u (log10($1)):2 pt 7 lc 0 lw 2 title "",\
"SED_data/1ES1741+196/Fermi.dat" every :::2::2 u (log10($1)):2:3 w filledcu lc rgb '#dddddd' lw 1 title "",\
"SED_data/1ES1741+196/Fermi.dat" every :::0::0 u (log10($1)):3:4 w yerrorbars pt 7 lc 8 lw 2 title "",\
"SED_data/1ES1741+196/Fermi.dat" every :::1::1 u (log10($1)):(1.5*$3):(0):(0.5*$3-$3) w vector lc 8 lw 2 title "",\
"SED_data/1ES1741+196/LAXPC_SED2_rebinned" u (log10($1)):2:3 w yerrorbars pt 7 lc 8 lw 2 title "",\
"SED_data/1ES1741+196/SXT_SED2_rebinned" u (log10($1)):2:3 w yerrorbars pt 7 lc 8 lw 2 title "",\
"SED_data/1ES1741+196/UVIT" u (log10($1)):2:3 w yerrorbars pt 7 lc 8 lw 2 title "",\
"steadystate/nFn_1741_2.dat" u (log10($1)):2 w l lc 7 lw 2 title "",\
"onehale/1741_2/Total_Power_lm.dat" u (log10($1)):3 w l lc 6 lw 2 dt (10,10) title "",\
"onehale/1741_2/Total_Power_hm.dat" u (log10($1)):3 w l lc 4 lw 2 dt (10,10,3,7) title "",\
"zech_model/HG_Costamante.dat" u (log10($1/(1+(0.084-0.184)))):($2*9.0) w l lc 0 lw 1 dt 1 title ""


unset multiplot





